A Kinematic Study of Wolf-Rayet Stars at the Galactic Center I: Binary Candidates and Constraints on the Binary Fraction

We report the binary fraction of Wolf-Rayet (WR) stars within 0.5~pc of the Galactic center obtained through the longest time-baseline (1994-2024) kinematic study of this population of stars. The new radial velocity ($v_{z}$) data we present is primarily from the W. M. Keck Observatory, with additional $v_{z}$ measurements from Gemini North Observatory. When combining our new $v_{z}$ measurements with literature measurements, we find $v_{z}$ variations suggesting the presence of a companion for five out of 27 WR stars, of which two are newly identified here (IRS~13E4, S8-181), along with three previously detected binaries (IRS~16SW, IRS~16NE, S4-258). Based on our experimental sensitivity and expected properties of the underlying population, we infer the binary fraction of the WR stars in the Galactic center to be 0.56$\pm$0.18. This is consistent with previous photometric studies of the young stars in the Galactic center, and with the binary fraction of field WR stars. When our results are combined with the results of previous photometric work, we find a binary fraction of 0.69$\pm$0.17 for the WR stars in the Galactic center.

==> aliases.tex <==

\begin{deluxetable}{cc}
\tablecolumns{2} 
\tablewidth{0pc}
\footnotesize
\tablecaption{Aliases of the Wolf-Rayet stars in the Galactic Center}
\tablehead{ 
	\colhead{Name} &
	\colhead{Aliases$^{a}$} \\
    \colhead{} &
    \colhead{} 
}
\startdata
IRS 16C & S96$^{1}$,E20$^{2}$ \\ 
IRS 16NW & E19$^{2}$  \\ 
IRS 16SW & S97$^{1}$,IRS 16SW(W)$^{3}$,E23$^{2}$ \\
 IRS 29N & E31$^{2}$ \\ 
IRS 16SW-E & E32$^{2}$,MPE +1.6-6.8$^{4}$ \\
S2-16 & E35$^{2}$,MPE-1.0-3.5$^{4}$ \\ 
IRS 16NE & E39$^{2}$ \\ 
S3-5 & E40$^{2}$,IRS 16SE2$^{5}$ \\ 
IRS 33E & E41$^{2}$ \\ 
IRS 13E4 & E48$^{2}$ \\ 
S3-12 & IRS 21$^{5}$ \\ 
IRS 13E2 & E51$^{2}$ \\ 
IRS 34W & E56$^{2}$ \\
IRS 3E & E58$^{2}$,IRS 3$^{5}$ \\
IRS 7SE & E59$^{2}$, [PMM2001] B9$^{6}$ \\ 
S4-258 & E60$^{2}$ \\ 
IRS 34NW & E61$^{2}$ \\ 
S4-342 & IRS 7SE2$^{5}$ \\
S5-69 & IRS 6E$^{5}$ \\ 
IRS 1W & E63$^{2}$ \\ 
IRS 9W & E65$^{2}$ \\ 
S6-90 & E66$^{2}$,IRS 7SW$^{5}$,WR1$^{8}$ \\ 
S6-95 & E68$^{2}$,IRS 7W$^{5}$,WR2$^{8}$ \\
S6-93 & E70$^{2}$,IRS 7E2$^{5}$,IRS 7ESE$^{5}$ \\ 
S6-100 & E71$^{2}$ \\ 
S6-82 & E72$^{2}$ \\ 
IRS 10W & \\ 
S8-181 & E74$^{2}$,AFNW$^{7}$ \\ 
S9-20 & E76$^{2}$,IRS 9SW$^{5}$ \\ 
S9-1 & E78$^{2}$,[PMM2001] B1$^{6}$ \\ 
S9-114 & E79$^{2}$,AF$^{7}$ \\ 
S9-283 & E81$^{2}$,AFNWNW$^{7}$ \\ 
S9-9 & E80$^{2}$,IRS 9SE$^{5}$ \\ 
S10-136 & E82$^{2}$,Blum$^{7}$ \\
S10-5 & E83$^{2}$,WR3$^{8}$ \\ 
S11-5 & E88$^{2}$ \\ 
IRS 5 & \\ 
\enddata
\tablenotetext{a}{Sources: 1) \citet{Eckart1997}, 2) \citet{Paumard2006}, 3) \citet{Zhu2008}, 4) \citet{Eckart1995}, 5) \citet{Bailey1984}, 6) \citet{Paumard2001}, 7) \citet{Genzel1996}, 8) \citet{Moultaka2005}}
\label{tab:aliases_table}
\end{deluxetable}
